The Platform Design Problem

On-line firms deploy suites of software platforms, where each platform is designed to interact with users during a certain activity, such as browsing, chatting, socializing, emailing, driving, etc. The economic and incentive structure of this exchange, as well as its algorithmic nature, have not been explored to our knowledge. We model this interaction as a Stackelberg game between a Designer and one or more Agents. We model an Agent as a Markov chain whose states are activities; we assume that the Agent's utility is a linear function of the steady-state distribution of this chain. The Designer may design a platform for each of these activities/states; if a platform is adopted by the Agent, the transition probabilities of the Markov chain are affected, and so is the objective of the Agent. The Designer's utility is a linear function of the steady state probabilities of the accessible states minus the development cost of the platforms. The underlying optimization problem of the Agent -- how to choose the states for which to adopt the platform -- is an MDP. If this MDP has a simple yet plausible structure (the transition probabilities from one state to another only depend on the target state and the recurrent probability of the current state) the Agent's problem can be solved by a greedy algorithm. The Designer's optimization problem (designing a custom suite for the Agent so as to optimize, through the Agent's optimum reaction, the Designer's revenue), is NP-hard to approximate within any finite ratio; however, the special case, while still NP-hard, has an FPTAS. These results generalize from a single Agent to a distribution of Agents with finite support, as well as to the setting where the Designer must find the best response to the existing strategies of other Designers. We discuss other implications of our results and directions of future research.

==> competition.tex <==
\section{Competition between Designers}
Many platform designers compete in the world today, and it is of great interest to study and understand the interaction of two or more platform designers with agents.  In this section (in summary) and continuing in the Appendix~\ref{appendixD} (in full detail), we confront the algorithmic problems involved in this extension of our model.

This is of course a Stackelberg game with two or more competing Stackelberg players.  First, it is not hard to argue that, at equilibrium, and since platform costs are positive, no two Designers will deploy a platform for the same state.  One immediate algorithmic problem (before asking about equilibria) is the {\em best response problem:} if a Designer is confronted with a situation in which other designers have already deployed several platforms at various states, which platforms should this Designer deploy?

To answer, we must first solve the {\em many platforms problem,} that is, the Agent's problem in the more general case when many platforms are available at eah state.  In the Appendix we develop such an algorithm (Algorithm 5), which solves this version of the Agent's problem in time $(O(n+m\log n)$, where $m$ is the total number of platforms.  The algorithm is a rather complex extension of the Greedy algorithm, using the same parameters $A,B$ and $z_j, \phi(j)$ for $j=1,\ldots,m$, and the associated function for the utility of a set $S$ of adopted platforms, $u(S)= \frac{A+\sum_{j \in S}z_j \phi(j) }{B + \sum_{j \in S} z_j}$.  The algorithm starts with a pass during which each platform is eliminated from further consideration if it satisfies any of three criteria. These criteria depend on the platform's $z_j$ and $\phi(j)$ values, and the values of the other platforms in the same state.  After the elimination phase, the algorithm considers the platforms in order of decreasing $\psi(j)$ (instead of $\phi(j)$ as in the single platform case), where $\psi$ is a function computed, through a planar convex geometry construction based on the $z_k$'s and $\phi(k)$'s of all platforms $k$ in the same state.  If the platform is the first one considered in the state, it is accepted in $S$.  If not, it replaces one particular platform in the same state that was already in $S$.  See the Appendix~\ref{appendixD} for full details.

Based on this algorithm, we develop in Appendix~\ref{sec.manyplatforms} an extension our algorithm for solving the Designer's problem for the case when other designers have already proposed platforms.  That is, the Designer must add to the mix its own optimum set of platforms such as the Agent, executing the algorithm described above, will end up choosing the optimum, from the point of view of the Designer, set of adopted platforms.  In other words, this solves the 

In Appendix~\ref{appendixD} we develop two algorithms that generalize those in the main paper to the competitive setting:  In Appendix~\ref{sec:agent-multiplatform} we develop an algorithm for the Agent's problem, when there are many platforms to choose from --- presumably, from many competing Designers. Based on this, we then develop, in Appendix~\ref{sec.manyplatforms}, an algorithm for the {\em best response} problem of a Designer when other designers have already deployed platforms.  Finally, in Appendix~\ref{appendixE} we show that a pure Nash equilibrium may not exist even in the flower setting. We conjecture that finding a pure equilibrium is $\Sigma_2$-complete, and we have some ideas about that proof.  But perhaps the most interesting strategic questions go beyond the model of this paper:  How are Designers incentivized by the competition to design and deploy platforms that are more beneficial to the Agents than in the monopolistic situation?

